OzSSy1: The Australian Southern Seyfert-1 Spectroscopic Atlas and Catalogue at $z<0.1$

We present a spectroscopic atlas of 1001 broad-line active galactic nuclei (AGNs) in the Southern sky, spanning redshifts $z < 0.1$, declinations $\delta < 0$ deg and Galactic latitudes $|b| > 10$ deg. The sample aims at being a comprehensive census of nearby broad-line AGNs at $K<13$ mag. The atlas is constructed from observations with $R\sim3000$ using the integral-field Wide Field Spectrograph at the Australian National University 2.3 m telescope. The data products include spectra, each accompanied by a spectral decomposition that models the AGN continuum and host galaxy, along with fits to the emission lines H$\gamma$, H$\beta$, H$\alpha$, He II, He I, [O III], [O I], [N II] and [S II], including broad Balmer and Helium components. The data products are publicly available and designed to support studies of population demographics and AGN variability in conjunction with future time-domain surveys.

==> output_arxiv.tex <==
\begin{thebibliography}{}
\makeatletter
\relax
\def\mn@urlcharsother{\let\do\@makeother \do\$\do\&\do\#\do\^\do\_\do\%\do\~}
\def\mn@doi{\begingroup\mn@urlcharsother \@ifnextchar [ {\mn@doi@} {\mn@doi@[]}}
\def\mn@doi@[#1]#2{\def\@tempa{#1}\ifx\@tempa\@empty \href {http://dx.doi.org/#2} {doi:#2}\else \href {http://dx.doi.org/#2} {#1}\fi \endgroup}
\def\mn@eprint#1#2{\mn@eprint@#1:#2::\@nil}
\def\mn@eprint@arXiv#1{\href {http://arxiv.org/abs/#1} {{\tt arXiv:#1}}}
\def\mn@eprint@dblp#1{\href {http://dblp.uni-trier.de/rec/bibtex/#1.xml} {dblp:#1}}
\def\mn@eprint@#1:#2:#3:#4\@nil{\def\@tempa {#1}\def\@tempb {#2}\def\@tempc {#3}\ifx \@tempc \@empty \let \@tempc \@tempb \let \@tempb \@tempa \fi \ifx \@tempb \@empty \def\@tempb {arXiv}\fi \@ifundefined {mn@eprint@\@tempb}{\@tempb:\@tempc}{\expandafter \expandafter \csname mn@eprint@\@tempb\endcsname \expandafter{\@tempc}}}

\bibitem[\protect\citeauthoryear{{Amrutha}}{{Amrutha}}{2026}]{pyspecextract_2026_v2}
{Amrutha} N.,  2026, PySpecExtract, \mn@doi{10.5281/zenodo.20741125}

\bibitem[\protect\citeauthoryear{{Amrutha}, {Wolf}, {Onken}, {Hon}, {Lai}, {Tonry}  \& {Webster}}{{Amrutha} et~al.}{2024}]{amrutha_wolf_2024}
{Amrutha} N.,  {Wolf} C.,  {Onken} C.~A.,  {Hon} W.~J.,  {Lai} S.,  {Tonry} J.~L.,   {Webster} R.,  2024, \mn@doi [\mnras] {10.1093/mnras/stae2470}, \href {https://ui.adsabs.harvard.edu/abs/2024MNRAS.535.2322A} {535, 2322}

\bibitem[\protect\citeauthoryear{{Amrutha}, {Wolf}, {Onken}, {Hon}, {Lai}, {Raithel}, {Tan}  \& {Webster}}{{Amrutha} et~al.}{2026}]{amrutha_masscorr_2026}
{Amrutha} N.,  {Wolf} C.,  {Onken} C.~A.,  {Hon} W.~J.,  {Lai} S.,  {Raithel} D.,  {Tan} A. H.~T.,   {Webster} R.,  2026, \mn@doi [Nature Communications] {10.1038/s41467-026-69166-w}

\bibitem[\protect\citeauthoryear{{Ar{\'e}valo}, {Churazov}, {Lira}, {S{\'a}nchez-S{\'a}ez}, {Bernal}, {Hern{\'a}ndez-Garc{\'\i}a}, {L{\'o}pez-Navas}  \& {Patel}}{{Ar{\'e}valo} et~al.}{2024}]{arevalo_churazov_2024}
{Ar{\'e}valo} P.,  {Churazov} E.,  {Lira} P.,  {S{\'a}nchez-S{\'a}ez} P.,  {Bernal} S.,  {Hern{\'a}ndez-Garc{\'\i}a} L.,  {L{\'o}pez-Navas} E.,   {Patel} P.,  2024, \mn@doi [\aap] {10.1051/0004-6361/202347080}, \href {https://ui.adsabs.harvard.edu/abs/2024A&A...684A.133A} {684, A133}

\bibitem[\protect\citeauthoryear{{Baldwin}}{{Baldwin}}{1977}]{baldwin_1977}
{Baldwin} J.~A.,  1977, \mn@doi [\apj] {10.1086/155294}, \href {https://ui.adsabs.harvard.edu/abs/1977ApJ...214..679B} {214, 679}

\bibitem[\protect\citeauthoryear{{Baldwin}, {Phillips}  \& {Terlevich}}{{Baldwin} et~al.}{1981}]{baldwin_phillips_BPT_1981}
{Baldwin} J.~A.,  {Phillips} M.~M.,   {Terlevich} R.,  1981, \mn@doi [\pasp] {10.1086/130766}, \href {https://ui.adsabs.harvard.edu/abs/1981PASP...93....5B} {93, 5}

\bibitem[\protect\citeauthoryear{{Barqu{\'\i}n-Gonz{\'a}lez} et~al.,}{{Barqu{\'\i}n-Gonz{\'a}lez} et~al.}{2024}]{barquingonzalez_mateos_2024}
{Barqu{\'\i}n-Gonz{\'a}lez} L.,  et~al., 2024, \mn@doi [\aap] {10.1051/0004-6361/202348948}, \href {https://ui.adsabs.harvard.edu/abs/2024A&A...687A.159B} {687, A159}

\bibitem[\protect\citeauthoryear{{Bauer}, {Condon}, {Thuan}  \& {Broderick}}{{Bauer} et~al.}{2000}]{bauer_condon_2000}
{Bauer} F.~E.,  {Condon} J.~J.,  {Thuan} T.~X.,   {Broderick} J.~J.,  2000, \mn@doi [\apjs] {10.1086/313425}, \href {https://ui.adsabs.harvard.edu/abs/2000ApJS..129..547B} {129, 547}

\bibitem[\protect\citeauthoryear{{Bellm} et~al.,}{{Bellm} et~al.}{2019}]{bellm_kulkarni_2019_ztf}
{Bellm} E.~C.,  et~al., 2019, \mn@doi [\pasp] {10.1088/1538-3873/aaecbe}, \href {https://ui.adsabs.harvard.edu/abs/2019PASP..131a8002B} {131, 018002}

\bibitem[\protect\citeauthoryear{{Bentz} et~al.,}{{Bentz} et~al.}{2010}]{bentz_walsh_2010}
{Bentz} M.~C.,  et~al., 2010, \mn@doi [\apj] {10.1088/0004-637X/716/2/993}, \href {https://ui.adsabs.harvard.edu/abs/2010ApJ...716..993B} {716, 993}

\bibitem[\protect\citeauthoryear{{Bianchi}, {Chiaberge}, {Laor}, {Antonucci}, {Bagul}  \& {Capetti}}{{Bianchi} et~al.}{2022}]{bianchi_chiaberge_2022_ngc3147}
{Bianchi} S.,  {Chiaberge} M.,  {Laor} A.,  {Antonucci} R.,  {Bagul} A.,   {Capetti} A.,  2022, \mn@doi [\mnras] {10.1093/mnras/stac2290}, \href {https://ui.adsabs.harvard.edu/abs/2022MNRAS.516.5775B} {516, 5775}

\bibitem[\protect\citeauthoryear{{Bikmaev}, {Sunyaev}, {Revnivtsev}  \& {Burenin}}{{Bikmaev} et~al.}{2006}]{bikmaev_sunyaev_2006}
{Bikmaev} I.~F.,  {Sunyaev} R.~A.,  {Revnivtsev} M.~G.,   {Burenin} R.~A.,  2006, \mn@doi [Astronomy Letters] {10.1134/S1063773706040013}, \href {https://ui.adsabs.harvard.edu/abs/2006AstL...32..221B} {32, 221}

\bibitem[\protect\citeauthoryear{{Blaes}, {Jiang}, {Lasota}  \& {Lipunova}}{{Blaes} et~al.}{2025}]{blaes_jiang_2025}
{Blaes} O.,  {Jiang} Y.-F.,  {Lasota} J.-P.,   {Lipunova} G.,  2025, \mn@doi [\ssr] {10.1007/s11214-025-01245-8}, \href {https://ui.adsabs.harvard.edu/abs/2025SSRv..221..120B} {221, 120}

\bibitem[\protect\citeauthoryear{{Blandford} \& {McKee}}{{Blandford} \& {McKee}}{1982}]{blandford_mckee_1982}
{Blandford} R.~D.,  {McKee} C.~F.,  1982, \mn@doi [\apj] {10.1086/159843}, \href {https://ui.adsabs.harvard.edu/abs/1982ApJ...255..419B} {255, 419}

\bibitem[\protect\citeauthoryear{{Bolton}, {Shimmins}  \& {Wall}}{{Bolton} et~al.}{1975}]{bolton_shimmins_1975}
{Bolton} J.~G.,  {Shimmins} A.~J.,   {Wall} J.~V.,  1975, Australian Journal of Physics Astrophysical Supplement, \href {https://ui.adsabs.harvard.edu/abs/1975AuJPA..34....1B} {34, 1}

\bibitem[\protect\citeauthoryear{{Bon} et~al.,}{{Bon} et~al.}{2016}]{bon_zucker_2016_ngc5548_lc}
{Bon} E.,  et~al., 2016, \mn@doi [\apjs] {10.3847/0067-0049/225/2/29}, \href {https://ui.adsabs.harvard.edu/abs/2016ApJS..225...29B} {225, 29}

\bibitem[\protect\citeauthoryear{{Bowen}, {Osmer}, {Blades}, {Tytler}, {Cottrell}, {Fan}  \& {Lanzetta}}{{Bowen} et~al.}{1994}]{bowen_osmer_1994}
{Bowen} D.~V.,  {Osmer} S.~J.,  {Blades} J.~C.,  {Tytler} D.,  {Cottrell} L.,  {Fan} X.-M.,   {Lanzetta} K.~M.,  1994, \mn@doi [\aj] {10.1086/116867}, \href {https://ui.adsabs.harvard.edu/abs/1994AJ....107..461B} {107, 461}

\bibitem[\protect\citeauthoryear{{Brown}, {Duncan}, {Landt}, {Kirk}, {Ricci}, {Kamraj}, {Salvato}  \& {Ananna}}{{Brown} et~al.}{2019}]{brown_duncan_2019}
{Brown} M.~J.~I.,  {Duncan} K.~J.,  {Landt} H.,  {Kirk} M.,  {Ricci} C.,  {Kamraj} N.,  {Salvato} M.,   {Ananna} T.,  2019, \mn@doi [\mnras] {10.1093/mnras/stz2324}, \href {https://ui.adsabs.harvard.edu/abs/2019MNRAS.489.3351B} {489, 3351}

\bibitem[\protect\citeauthoryear{{Cackett}, {Bentz}  \& {Kara}}{{Cackett} et~al.}{2021}]{cackett_bentz_2021}
{Cackett} E.~M.,  {Bentz} M.~C.,   {Kara} E.,  2021, \mn@doi [iScience] {10.1016/j.isci.2021.102557}, \href {https://ui.adsabs.harvard.edu/abs/2021iSci...24j2557C} {24, 102557}

\bibitem[\protect\citeauthoryear{{Calzetti}, {Armus}, {Bohlin}, {Kinney}, {Koornneef}  \& {Storchi-Bergmann}}{{Calzetti} et~al.}{2000}]{calzetti_armus_2000}
{Calzetti} D.,  {Armus} L.,  {Bohlin} R.~C.,  {Kinney} A.~L.,  {Koornneef} J.,   {Storchi-Bergmann} T.,  2000, \mn@doi [\apj] {10.1086/308692}, \href {https://ui.adsabs.harvard.edu/abs/2000ApJ...533..682C} {533, 682}

\bibitem[\protect\citeauthoryear{{Camus} \& {Panda}}{{Camus} \& {Panda}}{2026}]{camus_panda_2026}
{Camus} M.,  {Panda} S.,  2026, \mn@doi [arXiv e-prints] {10.48550/arXiv.2603.18255}, \href {https://ui.adsabs.harvard.edu/abs/2026arXiv260318255C} {p. arXiv:2603.18255}

\bibitem[\protect\citeauthoryear{{Chen}, {Zaw}, {Farrar}  \& {Elgamal}}{{Chen} et~al.}{2022}]{chen_zaw_2022}
{Chen} Y.-P.,  {Zaw} I.,  {Farrar} G.~R.,   {Elgamal} S.,  2022, \mn@doi [\apjs] {10.3847/1538-4365/ac4157}, \href {https://ui.adsabs.harvard.edu/abs/2022ApJS..258...29C} {258, 29}

\bibitem[\protect\citeauthoryear{{Chen} et~al.,}{{Chen} et~al.}{2023}]{chen_bao_2023}
{Chen} Y.-J.,  et~al., 2023, \mn@doi [\mnras] {10.1093/mnras/stad051}, \href {https://ui.adsabs.harvard.edu/abs/2023MNRAS.520.1807C} {520, 1807}

\bibitem[\protect\citeauthoryear{{Childress}, {Vogt}, {Nielsen}  \& {Sharp}}{{Childress} et~al.}{2014}]{childress_vogt_2014_pywifes}
{Childress} M.~J.,  {Vogt} F. P.~A.,  {Nielsen} J.,   {Sharp} R.~G.,  2014, \mn@doi [\apss] {10.1007/s10509-013-1682-0}, \href {https://ui.adsabs.harvard.edu/abs/2014Ap&SS.349..617C} {349, 617}

\bibitem[\protect\citeauthoryear{{Cho} et~al.,}{{Cho} et~al.}{2023}]{cho_woo_2023_halpha_mass}
{Cho} H.,  et~al., 2023, \mn@doi [\apj] {10.3847/1538-4357/ace1e5}, \href {https://ui.adsabs.harvard.edu/abs/2023ApJ...953..142C} {953, 142}

\bibitem[\protect\citeauthoryear{{Colless} et~al.,}{{Colless} et~al.}{2001}]{colless_dalton_2001}
{Colless} M.,  et~al., 2001, \mn@doi [\mnras] {10.1046/j.1365-8711.2001.04902.x}, \href {https://ui.adsabs.harvard.edu/abs/2001MNRAS.328.1039C} {328, 1039}

\bibitem[\protect\citeauthoryear{{Crenshaw}, {Kraemer}  \& {Gabel}}{{Crenshaw} et~al.}{2003}]{crenshaw_kraemer_2003}
{Crenshaw} D.~M.,  {Kraemer} S.~B.,   {Gabel} J.~R.,  2003, \mn@doi [\aj] {10.1086/377625}, \href {https://ui.adsabs.harvard.edu/abs/2003AJ....126.1690C} {126, 1690}

\bibitem[\protect\citeauthoryear{{DESI Collaboration} et~al.,}{{DESI Collaboration} et~al.}{2026}]{desi_dr1}
{DESI Collaboration} et~al., 2026, \mn@doi [\aj] {10.3847/1538-3881/ae4c43}, \href {https://ui.adsabs.harvard.edu/abs/2026AJ....171..285D} {171, 285}

\bibitem[\protect\citeauthoryear{{Dopita} \& {Sutherland}}{{Dopita} \& {Sutherland}}{2003}]{dopita_sutherland_2003}
{Dopita} M.~A.,  {Sutherland} R.~S.,  2003, {Astrophysics of the diffuse universe}.
Springer, \mn@doi{10.1007/978-3-662-05866-4}

\bibitem[\protect\citeauthoryear{{Dopita}, {Hart}, {McGregor}, {Oates}, {Bloxham}  \& {Jones}}{{Dopita} et~al.}{2007}]{dopita_hart_2007}
{Dopita} M.,  {Hart} J.,  {McGregor} P.,  {Oates} P.,  {Bloxham} G.,   {Jones} D.,  2007, \mn@doi [\apss] {10.1007/s10509-007-9510-z}, \href {https://ui.adsabs.harvard.edu/abs/2007Ap&SS.310..255D} {310, 255}

\bibitem[\protect\citeauthoryear{{Dopita} et~al.,}{{Dopita} et~al.}{2010}]{dopita_rhee_2010}
{Dopita} M.,  et~al., 2010, \mn@doi [\apss] {10.1007/s10509-010-0335-9}, \href {https://ui.adsabs.harvard.edu/abs/2010Ap&SS.327..245D} {327, 245}

\bibitem[\protect\citeauthoryear{{Feng}, {Shen}  \& {Li}}{{Feng} et~al.}{2014}]{feng_shen_li_2014_l5100_mass}
{Feng} H.,  {Shen} Y.,   {Li} H.,  2014, \mn@doi [\apj] {10.1088/0004-637X/794/1/77}, \href {https://ui.adsabs.harvard.edu/abs/2014ApJ...794...77F} {794, 77}

\bibitem[\protect\citeauthoryear{{Flesch}}{{Flesch}}{2023}]{milliquas_2023}
{Flesch} E.~W.,  2023, \mn@doi [The Open Journal of Astrophysics] {10.21105/astro.2308.01505}, \href {https://ui.adsabs.harvard.edu/abs/2023OJAp....6E..49F} {6, 49}

\bibitem[\protect\citeauthoryear{{Fries} et~al.,}{{Fries} et~al.}{2024}]{fries_trump_2024}
{Fries} L.~B.,  et~al., 2024, \mn@doi [\apj] {10.3847/1538-4357/ad7c42}, \href {https://ui.adsabs.harvard.edu/abs/2024ApJ...975..239F} {975, 239}

\bibitem[\protect\citeauthoryear{{Gaia Collaboration} et~al.,}{{Gaia Collaboration} et~al.}{2023}]{gaia_dr3}
{Gaia Collaboration} et~al., 2023, \mn@doi [\aap] {10.1051/0004-6361/202243940}, \href {https://ui.adsabs.harvard.edu/abs/2023A&A...674A...1G} {674, A1}

\bibitem[\protect\citeauthoryear{{Gaskell}}{{Gaskell}}{2017}]{martin_2017_caseB}
{Gaskell} C.~M.,  2017, \mn@doi [\mnras] {10.1093/mnras/stx094}, \href {https://ui.adsabs.harvard.edu/abs/2017MNRAS.467..226G} {467, 226}

\bibitem[\protect\citeauthoryear{{Gezari}}{{Gezari}}{2021}]{gezari_tde_2021}
{Gezari} S.,  2021, \mn@doi [\araa] {10.1146/annurev-astro-111720-030029}, \href {https://ui.adsabs.harvard.edu/abs/2021ARA&A..59...21G} {59, 21}

\bibitem[\protect\citeauthoryear{{Grazian}, {Omizzolo}, {Corbally}, {Cristiani}, {Haehnelt}  \& {Vanzella}}{{Grazian} et~al.}{2002}]{grazian_omizzolo_2002}
{Grazian} A.,  {Omizzolo} A.,  {Corbally} C.,  {Cristiani} S.,  {Haehnelt} M.~G.,   {Vanzella} E.,  2002, \mn@doi [\aj] {10.1086/343834}, \href {https://ui.adsabs.harvard.edu/abs/2002AJ....124.2955G} {124, 2955}

\bibitem[\protect\citeauthoryear{{Greene} et~al.,}{{Greene} et~al.}{2010}]{greene_hood_2010_oiii_RL}
{Greene} J.~E.,  et~al., 2010, \mn@doi [\apj] {10.1088/0004-637X/723/1/409}, \href {https://ui.adsabs.harvard.edu/abs/2010ApJ...723..409G} {723, 409}

\bibitem[\protect\citeauthoryear{{Ho}}{{Ho}}{2008}]{ho_2008_rev}
{Ho} L.~C.,  2008, \mn@doi [\araa] {10.1146/annurev.astro.45.051806.110546}, \href {https://ui.adsabs.harvard.edu/abs/2008ARA&A..46..475H} {46, 475}

\bibitem[\protect\citeauthoryear{{Ho}, {Filippenko}  \& {Sargent}}{{Ho} et~al.}{1997}]{ho_filippenko_1997}
{Ho} L.~C.,  {Filippenko} A.~V.,   {Sargent} W. L.~W.,  1997, \mn@doi [\apj] {10.1086/304638}, \href {https://ui.adsabs.harvard.edu/abs/1997ApJ...487..568H} {487, 568}

\bibitem[\protect\citeauthoryear{{Hon}, {Wolf}, {Onken}, {Webster}  \& {Auchettl}}{{Hon} et~al.}{2022}]{hon_wolf_2022_skymapper_colors}
{Hon} W.~J.,  {Wolf} C.,  {Onken} C.~A.,  {Webster} R.,   {Auchettl} K.,  2022, \mn@doi [\mnras] {10.1093/mnras/stab3694}, \href {https://ui.adsabs.harvard.edu/abs/2022MNRAS.511...54H} {511, 54}

\bibitem[\protect\citeauthoryear{{Hon}, {Webster}  \& {Wolf}}{{Hon} et~al.}{2025}]{hon_webster_2025}
{Hon} W.~J.,  {Webster} R.~L.,   {Wolf} C.,  2025, \mn@doi [\mnras] {10.1093/mnras/stae2815}, \href {https://ui.adsabs.harvard.edu/abs/2025MNRAS.536.3611H} {536, 3611}

\bibitem[\protect\citeauthoryear{{Huchra} et~al.,}{{Huchra} et~al.}{2012}]{huchra_macri_2012}
{Huchra} J.~P.,  et~al., 2012, \mn@doi [\apjs] {10.1088/0067-0049/199/2/26}, \href {https://ui.adsabs.harvard.edu/abs/2012ApJS..199...26H} {199, 26}

\bibitem[\protect\citeauthoryear{{Ivezi{\'c}} et~al.,}{{Ivezi{\'c}} et~al.}{2019}]{LSST_plan}
{Ivezi{\'c}} {\v{Z}}.,  et~al., 2019, \mn@doi [\apj] {10.3847/1538-4357/ab042c}, \href {https://ui.adsabs.harvard.edu/abs/2019ApJ...873..111I} {873, 111}

\bibitem[\protect\citeauthoryear{{Jarrett}, {Chester}, {Cutri}, {Schneider}, {Rosenberg}, {Huchra}  \& {Mader}}{{Jarrett} et~al.}{2000}]{jarrett_chester_2000}
{Jarrett} T.~H.,  {Chester} T.,  {Cutri} R.,  {Schneider} S.,  {Rosenberg} J.,  {Huchra} J.~P.,   {Mader} J.,  2000, \mn@doi [\aj] {10.1086/301426}, \href {https://ui.adsabs.harvard.edu/abs/2000AJ....120..298J} {120, 298}

\bibitem[\protect\citeauthoryear{{Jones} et~al.,}{{Jones} et~al.}{2004}]{jones_saunders_2004_6dfgs}
{Jones} D.~H.,  et~al., 2004, \mn@doi [\mnras] {10.1111/j.1365-2966.2004.08353.x}, \href {https://ui.adsabs.harvard.edu/abs/2004MNRAS.355..747J} {355, 747}

\bibitem[\protect\citeauthoryear{{Jones} et~al.,}{{Jones} et~al.}{2009}]{jones_read_2009_6dfgs}
{Jones} D.~H.,  et~al., 2009, \mn@doi [\mnras] {10.1111/j.1365-2966.2009.15338.x}, \href {https://ui.adsabs.harvard.edu/abs/2009MNRAS.399..683J} {399, 683}

\bibitem[\protect\citeauthoryear{{Kauffmann} et~al.,}{{Kauffmann} et~al.}{2003}]{kauffmann_heckman_2003}
{Kauffmann} G.,  et~al., 2003, \mn@doi [\mnras] {10.1111/j.1365-2966.2003.07154.x}, \href {https://ui.adsabs.harvard.edu/abs/2003MNRAS.346.1055K} {346, 1055}

\bibitem[\protect\citeauthoryear{{Kelly}, {Bechtold}  \& {Siemiginowska}}{{Kelly} et~al.}{2009}]{kelly_bechtold_2009}
{Kelly} B.~C.,  {Bechtold} J.,   {Siemiginowska} A.,  2009, \mn@doi [\apj] {10.1088/0004-637X/698/1/895}, \href {https://ui.adsabs.harvard.edu/abs/2009ApJ...698..895K} {698, 895}

\bibitem[\protect\citeauthoryear{{Kewley}, {Heisler}, {Dopita}  \& {Lumsden}}{{Kewley} et~al.}{2001}]{kewley_heisler_2001}
{Kewley} L.~J.,  {Heisler} C.~A.,  {Dopita} M.~A.,   {Lumsden} S.,  2001, \mn@doi [\apjs] {10.1086/318944}, \href {https://ui.adsabs.harvard.edu/abs/2001ApJS..132...37K} {132, 37}

\bibitem[\protect\citeauthoryear{{Kewley}, {Groves}, {Kauffmann}  \& {Heckman}}{{Kewley} et~al.}{2006}]{kewley_groves_2006}
{Kewley} L.~J.,  {Groves} B.,  {Kauffmann} G.,   {Heckman} T.,  2006, \mn@doi [\mnras] {10.1111/j.1365-2966.2006.10859.x}, \href {https://ui.adsabs.harvard.edu/abs/2006MNRAS.372..961K} {372, 961}

\bibitem[\protect\citeauthoryear{{Kollatschny}, {Kotulla}, {Pietsch}, {Bischoff}  \& {Zetzl}}{{Kollatschny} et~al.}{2008}]{kollatchny_kotulla_2008}
{Kollatschny} W.,  {Kotulla} R.,  {Pietsch} W.,  {Bischoff} K.,   {Zetzl} M.,  2008, \mn@doi [\aap] {10.1051/0004-6361:20078552}, \href {https://ui.adsabs.harvard.edu/abs/2008A&A...484..897K} {484, 897}

\bibitem[\protect\citeauthoryear{{Kollmeier} et~al.,}{{Kollmeier} et~al.}{2026}]{kollmeier_rix_2026_SDSSV}
{Kollmeier} J.~A.,  et~al., 2026, \mn@doi [\aj] {10.3847/1538-3881/ae0576}, \href {https://ui.adsabs.harvard.edu/abs/2026AJ....171...52K} {171, 52}

\bibitem[\protect\citeauthoryear{{Konig}, {Staubert}  \& {Geckeler}}{{Konig} et~al.}{1998}]{konig_staubert_1998}
{Konig} M.,  {Staubert} R.,   {Geckeler} R.,  1998, \aap, \href {https://ui.adsabs.harvard.edu/abs/1998A&A...329...68K} {329, 68}

\bibitem[\protect\citeauthoryear{{Kova{\v{c}}evi{\'c}-Doj{\v{c}}inovi{\'c}}, {Doj{\v{c}}inovi{\'c}}, {Laki{\'c}evi{\'c}}  \& {Popovi{\'c}}}{{Kova{\v{c}}evi{\'c}-Doj{\v{c}}inovi{\'c}} et~al.}{2022}]{kovacevic_dojcinovic_2022}
{Kova{\v{c}}evi{\'c}-Doj{\v{c}}inovi{\'c}} J.,  {Doj{\v{c}}inovi{\'c}} I.,  {Laki{\'c}evi{\'c}} M.,   {Popovi{\'c}} L.~{\v{C}}.,  2022, \mn@doi [\aap] {10.1051/0004-6361/202141043}, \href {https://ui.adsabs.harvard.edu/abs/2022A&A...659A.130K} {659, A130}

\bibitem[\protect\citeauthoryear{{Lamontagne}, {Demers}, {Wesemael}, {Fontaine}  \& {Irwin}}{{Lamontagne} et~al.}{2000}]{lamontagne_demers_2000}
{Lamontagne} R.,  {Demers} S.,  {Wesemael} F.,  {Fontaine} G.,   {Irwin} M.~J.,  2000, \mn@doi [\aj] {10.1086/301181}, \href {https://ui.adsabs.harvard.edu/abs/2000AJ....119..241L} {119, 241}

\bibitem[\protect\citeauthoryear{{Lawrence} et~al.,}{{Lawrence} et~al.}{2016}]{lawrence_bruce_2016}
{Lawrence} A.,  et~al., 2016, \mn@doi [\mnras] {10.1093/mnras/stw1963}, \href {https://ui.adsabs.harvard.edu/abs/2016MNRAS.463..296L} {463, 296}

\bibitem[\protect\citeauthoryear{{Liu}, {Liu}, {Dong}, {Zhou}, {Wang}, {Lu}  \& {Yuan}}{{Liu} et~al.}{2019}]{liu_liu_2019_lozagn}
{Liu} H.-Y.,  {Liu} W.-J.,  {Dong} X.-B.,  {Zhou} H.,  {Wang} T.,  {Lu} H.,   {Yuan} W.,  2019, \mn@doi [\apjs] {10.3847/1538-4365/ab298b}, \href {https://ui.adsabs.harvard.edu/abs/2019ApJS..243...21L} {243, 21}

\bibitem[\protect\citeauthoryear{{L{\'o}pez-Navas} et~al.,}{{L{\'o}pez-Navas} et~al.}{2022}]{lopez_martinez_2022}
{L{\'o}pez-Navas} E.,  et~al., 2022, \mn@doi [\mnras] {10.1093/mnrasl/slac033}, \href {https://ui.adsabs.harvard.edu/abs/2022MNRAS.513L..57L} {513, L57}

\bibitem[\protect\citeauthoryear{{L{\'o}pez-Navas} et~al.,}{{L{\'o}pez-Navas} et~al.}{2023}]{lopez-navas_sanchez-saez_2023}
{L{\'o}pez-Navas} E.,  et~al., 2023, \mn@doi [\mnras] {10.1093/mnras/stad1893}, \href {https://ui.adsabs.harvard.edu/abs/2023MNRAS.524..188L} {524, 188}

\bibitem[\protect\citeauthoryear{{MacLeod} et~al.,}{{MacLeod} et~al.}{2016}]{macleod_ross_2016}
{MacLeod} C.~L.,  et~al., 2016, \mn@doi [\mnras] {10.1093/mnras/stv2997}, \href {https://ui.adsabs.harvard.edu/abs/2016MNRAS.457..389M} {457, 389}

\bibitem[\protect\citeauthoryear{{MacLeod} et~al.,}{{MacLeod} et~al.}{2019}]{macleod_green_2019}
{MacLeod} C.~L.,  et~al., 2019, \mn@doi [\apj] {10.3847/1538-4357/ab05e2}, \href {https://ui.adsabs.harvard.edu/abs/2019ApJ...874....8M} {874, 8}

\bibitem[\protect\citeauthoryear{{Maia}, {Machado}  \& {Willmer}}{{Maia} et~al.}{2003}]{maia_machado_2003}
{Maia} M. A.~G.,  {Machado} R.~S.,   {Willmer} C. N.~A.,  2003, \mn@doi [\aj] {10.1086/378360}, \href {https://ui.adsabs.harvard.edu/abs/2003AJ....126.1750M} {126, 1750}

\bibitem[\protect\citeauthoryear{{Malyali} et~al.,}{{Malyali} et~al.}{2024}]{malyali_rau_2024}
{Malyali} A.,  et~al., 2024, \mn@doi [\mnras] {10.1093/mnras/stae927}, \href {https://ui.adsabs.harvard.edu/abs/2024MNRAS.531.1256M} {531, 1256}

\bibitem[\protect\citeauthoryear{{Markaryan} \& {Lipovetskii}}{{Markaryan} \& {Lipovetskii}}{1973}]{markaryan_lipovetskii_1973}
{Markaryan} B.~E.,  {Lipovetskii} V.~A.,  1973, \mn@doi [Astrophysics] {10.1007/BF01002512}, \href {https://ui.adsabs.harvard.edu/abs/1973Ap......9..283M} {9, 283}

\bibitem[\protect\citeauthoryear{{Marocco} et~al.,}{{Marocco} et~al.}{2021}]{marocco_eisenhardt_catwise_2021}
{Marocco} F.,  et~al., 2021, \mn@doi [\apjs] {10.3847/1538-4365/abd805}, \href {https://ui.adsabs.harvard.edu/abs/2021ApJS..253....8M} {253, 8}

\bibitem[\protect\citeauthoryear{{Mathewson}, {Hart}, {Wehner}, {Hovey}  \& {van Harmelen}}{{Mathewson} et~al.}{2013}]{mathewson_hart_2013}
{Mathewson} D.~S.,  {Hart} J.,  {Wehner} H.~P.,  {Hovey} G.~R.,   {van Harmelen} J.,  2013, Journal of Astronomical History and Heritage, \href {https://ui.adsabs.harvard.edu/abs/2013JAHH...16....2M} {16, 2}

\bibitem[\protect\citeauthoryear{{Mauch} \& {Sadler}}{{Mauch} \& {Sadler}}{2007}]{mauch_sadler_2007}
{Mauch} T.,  {Sadler} E.~M.,  2007, \mn@doi [\mnras] {10.1111/j.1365-2966.2006.11353.x}, \href {https://ui.adsabs.harvard.edu/abs/2007MNRAS.375..931M} {375, 931}

\bibitem[\protect\citeauthoryear{{Mazzarella} \& {Boroson}}{{Mazzarella} \& {Boroson}}{1993}]{mazzarella_boroson_1993}
{Mazzarella} J.~M.,  {Boroson} T.~A.,  1993, \mn@doi [\apjs] {10.1086/191754}, \href {https://ui.adsabs.harvard.edu/abs/1993ApJS...85...27M} {85, 27}

\bibitem[\protect\citeauthoryear{{McIntosh}, {Bell}, {Weinberg}  \& {Katz}}{{McIntosh} et~al.}{2006}]{mcintosh_bell_2006}
{McIntosh} D.~H.,  {Bell} E.~F.,  {Weinberg} M.~D.,   {Katz} N.,  2006, \mn@doi [\mnras] {10.1111/j.1365-2966.2006.11115.x}, \href {https://ui.adsabs.harvard.edu/abs/2006MNRAS.373.1321M} {373, 1321}

\bibitem[\protect\citeauthoryear{{McMahon}, {Banerji}, {Gonzalez}, {Koposov}, {Bejar}, {Lodieu}, {Rebolo}  \& {VHS Collaboration}}{{McMahon} et~al.}{2013}]{mcmahon_banerji_vhs_2013}
{McMahon} R.~G.,  {Banerji} M.,  {Gonzalez} E.,  {Koposov} S.~E.,  {Bejar} V.~J.,  {Lodieu} N.,  {Rebolo} R.,   {VHS Collaboration} 2013, The Messenger, \href {https://ui.adsabs.harvard.edu/abs/2013Msngr.154...35M} {154, 35}

\bibitem[\protect\citeauthoryear{{McMahon}, {Banerji}, {Gonzalez}, {Koposov}, {Bejar}, {Lodieu}, {Rebolo}  \& {VHS Collaboration}}{{McMahon} et~al.}{2021}]{vhs_dr5_cat_2021}
{McMahon} R.~G.,  {Banerji} M.,  {Gonzalez} E.,  {Koposov} S.~E.,  {Bejar} V.~J.,  {Lodieu} N.,  {Rebolo} R.,   {VHS Collaboration} 2021, {VizieR Online Data Catalog: The VISTA Hemisphere Survey (VHS) catalog DR5 (McMahon+, 2020)}, VizieR On-line Data Catalog: II/367. Originally published in: 2013Msngr.154...35M

\bibitem[\protect\citeauthoryear{{Monroe}, {Prochaska}, {Tejos}, {Worseck}, {Hennawi}, {Schmidt}, {Tumlinson}  \& {Shen}}{{Monroe} et~al.}{2016}]{monroe_prochaska_2016}
{Monroe} T.~R.,  {Prochaska} J.~X.,  {Tejos} N.,  {Worseck} G.,  {Hennawi} J.~F.,  {Schmidt} T.,  {Tumlinson} J.,   {Shen} Y.,  2016, \mn@doi [\aj] {10.3847/0004-6256/152/1/25}, \href {https://ui.adsabs.harvard.edu/abs/2016AJ....152...25M} {152, 25}

\bibitem[\protect\citeauthoryear{{Oh} et~al.,}{{Oh} et~al.}{2022}]{oh_koss_2022}
{Oh} K.,  et~al., 2022, \mn@doi [\apjs] {10.3847/1538-4365/ac5b68}, \href {https://ui.adsabs.harvard.edu/abs/2022ApJS..261....4O} {261, 4}

\bibitem[\protect\citeauthoryear{{Onken}, {Wolf}, {Hon}, {Lai}, {Tisserand}  \& {Webster}}{{Onken} et~al.}{2023}]{onken_wolf_AllBRICQS_2023}
{Onken} C.~A.,  {Wolf} C.,  {Hon} W.~J.,  {Lai} S.,  {Tisserand} P.,   {Webster} R.,  2023, \mn@doi [\pasa] {10.1017/pasa.2023.7}, \href {https://ui.adsabs.harvard.edu/abs/2023PASA...40...10O} {40, e010}

\bibitem[\protect\citeauthoryear{{Onken}, {Wolf}, {Bessell}, {Chang}, {Luvaul}, {Tonry}, {White}  \& {Da Costa}}{{Onken} et~al.}{2024}]{onken_wolf_2024_smssdr4}
{Onken} C.~A.,  {Wolf} C.,  {Bessell} M.~S.,  {Chang} S.-W.,  {Luvaul} L.~C.,  {Tonry} J.~L.,  {White} M.~C.,   {Da Costa} G.~S.,  2024, \mn@doi [\pasa] {10.1017/pasa.2024.53}, \href {https://ui.adsabs.harvard.edu/abs/2024PASA...41...61O} {41, e061}

\bibitem[\protect\citeauthoryear{{Paturel}, {Petit}, {Prugniel}, {Theureau}, {Rousseau}, {Brouty}, {Dubois}  \& {Cambr{\'e}sy}}{{Paturel} et~al.}{2003}]{paturel_petit_2003_pgc}
{Paturel} G.,  {Petit} C.,  {Prugniel} P.,  {Theureau} G.,  {Rousseau} J.,  {Brouty} M.,  {Dubois} P.,   {Cambr{\'e}sy} L.,  2003, \mn@doi [\aap] {10.1051/0004-6361:20031411}, \href {https://ui.adsabs.harvard.edu/abs/2003A&A...412...45P} {412, 45}

\bibitem[\protect\citeauthoryear{{Peterson} et~al.,}{{Peterson} et~al.}{2004}]{peterson_ferrarese_2004}
{Peterson} B.~M.,  et~al., 2004, \mn@doi [\apj] {10.1086/423269}, \href {https://ui.adsabs.harvard.edu/abs/2004ApJ...613..682P} {613, 682}

\bibitem[\protect\citeauthoryear{{Planck Collaboration} et~al.,}{{Planck Collaboration} et~al.}{2016}]{planck_gnilc_dust_2016}
{Planck Collaboration} et~al., 2016, \mn@doi [\aap] {10.1051/0004-6361/201629022}, \href {https://ui.adsabs.harvard.edu/abs/2016A&A...596A.109P} {596, A109}

\bibitem[\protect\citeauthoryear{{Price}, {Nielsen}, {Lidman}, {Soon}, {Travouillon}  \& {Sharp}}{{Price} et~al.}{2024}]{price_nielsen_robotic_2024}
{Price} I.,  {Nielsen} J.,  {Lidman} C.,  {Soon} J.,  {Travouillon} T.,   {Sharp} R.,  2024, \mn@doi [\pasa] {10.1017/pasa.2024.75}, \href {https://ui.adsabs.harvard.edu/abs/2024PASA...41...57P} {41, e057}

\bibitem[\protect\citeauthoryear{{Rakshit}, {Stalin}  \& {Kotilainen}}{{Rakshit} et~al.}{2020}]{rakshit_stalin_2020}
{Rakshit} S.,  {Stalin} C.~S.,   {Kotilainen} J.,  2020, \mn@doi [\apjs] {10.3847/1538-4365/ab99c5}, \href {https://ui.adsabs.harvard.edu/abs/2020ApJS..249...17R} {249, 17}

\bibitem[\protect\citeauthoryear{{Ricci} \& {Trakhtenbrot}}{{Ricci} \& {Trakhtenbrot}}{2023}]{ricci_trakhtenbrot_2022}
{Ricci} C.,  {Trakhtenbrot} B.,  2023, \mn@doi [Nature Astronomy] {10.1038/s41550-023-02108-4}, \href {https://ui.adsabs.harvard.edu/abs/2023NatAs...7.1282R} {7, 1282}

\bibitem[\protect\citeauthoryear{{SDSS Collaboration} et~al.,}{{SDSS Collaboration} et~al.}{2026}]{sdss_dr20}
{SDSS Collaboration} et~al., 2026, \mn@doi [arXiv e-prints] {10.48550/arXiv.2607.26149}, \href {https://ui.adsabs.harvard.edu/abs/2026arXiv260726149S} {p. arXiv:2607.26149}

\bibitem[\protect\citeauthoryear{{Saha} et~al.,}{{Saha} et~al.}{2025}]{saha_markowitz_2025}
{Saha} T.,  et~al., 2025, \mn@doi [\aap] {10.1051/0004-6361/202347985}, \href {https://ui.adsabs.harvard.edu/abs/2025A&A...702A..28S} {702, A28}

\bibitem[\protect\citeauthoryear{{S{\'a}nchez-S{\'a}ez} et~al.,}{{S{\'a}nchez-S{\'a}ez} et~al.}{2024}]{sanchez-saez_hernandez_2024_varOIII}
{S{\'a}nchez-S{\'a}ez} P.,  et~al., 2024, \mn@doi [\aap] {10.1051/0004-6361/202347957}, \href {https://ui.adsabs.harvard.edu/abs/2024A&A...688A.157S} {688, A157}

\bibitem[\protect\citeauthoryear{{Sandage} \& {Bedke}}{{Sandage} \& {Bedke}}{1994}]{sandage_bedke_1994}
{Sandage} A.,  {Bedke} J.,  1994, {The Carnegie atlas of galaxies}.
 I, II., Vol. 638, Carnegie Institution of Washington Publ.

\bibitem[\protect\citeauthoryear{{Sanders}, {Mazzarella}, {Kim}, {Surace}  \& {Soifer}}{{Sanders} et~al.}{2003}]{sanders_mazzarella_2003}
{Sanders} D.~B.,  {Mazzarella} J.~M.,  {Kim} D.-C.,  {Surace} J.~A.,   {Soifer} B.~T.,  2003, \mn@doi [\aj] {10.1086/376841}, \href {https://ui.adsabs.harvard.edu/abs/2003AJ....126.1607S} {126, 1607}

\bibitem[\protect\citeauthoryear{{Schlafly} \& {Finkbeiner}}{{Schlafly} \& {Finkbeiner}}{2011}]{dust_map_SandF_2011}
{Schlafly} E.~F.,  {Finkbeiner} D.~P.,  2011, \mn@doi [\apj] {10.1088/0004-637X/737/2/103}, \href {https://ui.adsabs.harvard.edu/abs/2011ApJ...737..103S} {737, 103}

\bibitem[\protect\citeauthoryear{{Schwope} et~al.,}{{Schwope} et~al.}{2000}]{schwope_hasinger_2000}
{Schwope} A.,  et~al., 2000, \mn@doi [Astronomische Nachrichten] {10.1002/(SICI)1521-3994(200003)321:1<1::AID-ASNA1>3.0.CO;2-C}, \href {https://ui.adsabs.harvard.edu/abs/2000AN....321....1S} {321, 1}

\bibitem[\protect\citeauthoryear{{Sexton}, {Matzko}, {Darden}, {Canalizo}  \& {Gorjian}}{{Sexton} et~al.}{2021}]{sexton_matzko_2021_badass3}
{Sexton} R.~O.,  {Matzko} W.,  {Darden} N.,  {Canalizo} G.,   {Gorjian} V.,  2021, \mn@doi [\mnras] {10.1093/mnras/staa3278}, \href {https://ui.adsabs.harvard.edu/abs/2021MNRAS.500.2871S} {500, 2871}

\bibitem[\protect\citeauthoryear{{Seyfert}}{{Seyfert}}{1943}]{seyfert_1943}
{Seyfert} C.~K.,  1943, \mn@doi [\apj] {10.1086/144488}, \href {https://ui.adsabs.harvard.edu/abs/1943ApJ....97...28S} {97, 28}

\bibitem[\protect\citeauthoryear{{Shen} et~al.,}{{Shen} et~al.}{2019}]{shen_hall_2019}
{Shen} Y.,  et~al., 2019, \mn@doi [\apjs] {10.3847/1538-4365/ab074f}, \href {https://ui.adsabs.harvard.edu/abs/2019ApJS..241...34S} {241, 34}

\bibitem[\protect\citeauthoryear{{Suresh}, {Hon}, {Webster}, {Wolf}  \& {Onken}}{{Suresh} et~al.}{2025}]{suresh_hon_2025}
{Suresh} S.,  {Hon} W.~J.,  {Webster} R.~L.,  {Wolf} C.,   {Onken} C.~A.,  2025, \mn@doi [\mnras] {10.1093/mnras/staf1591}, \href {https://ui.adsabs.harvard.edu/abs/2025MNRAS.543.3649S} {543, 3649}

\bibitem[\protect\citeauthoryear{{Tan}, {Wolf}, {Amrutha}, {Onken}, {Tonry}  \& {Webster}}{{Tan} et~al.}{2026}]{tan_wolf_2026}
{Tan} A. H.~T.,  {Wolf} C.,  {Amrutha} N.,  {Onken} C.~A.,  {Tonry} J.~L.,   {Webster} R.,  2026, \mn@doi [arXiv e-prints] {10.48550/arXiv.2605.03577}, \href {https://ui.adsabs.harvard.edu/abs/2026arXiv260503577T} {p. arXiv:2605.03577}

\bibitem[\protect\citeauthoryear{{Tang}, {Wolf}  \& {Tonry}}{{Tang} et~al.}{2023}]{tang_wolf_2023}
{Tang} J.-J.,  {Wolf} C.,   {Tonry} J.,  2023, \mn@doi [Nature Astronomy] {10.1038/s41550-022-01885-8}, \href {https://ui.adsabs.harvard.edu/abs/2023NatAs...7..473T} {7, 473}

\bibitem[\protect\citeauthoryear{{Taylor} et~al.,}{{Taylor} et~al.}{2023}]{taylor_cluver_2023}
{Taylor} E.~N.,  et~al., 2023, \mn@doi [The Messenger] {10.18727/0722-6691/5312}, \href {https://ui.adsabs.harvard.edu/abs/2023Msngr.190...46T} {190, 46}

\bibitem[\protect\citeauthoryear{{Thomas} et~al.,}{{Thomas} et~al.}{2017}]{thomas_dopita_2017}
{Thomas} A.~D.,  et~al., 2017, \mn@doi [\apjs] {10.3847/1538-4365/aa855a}, \href {https://ui.adsabs.harvard.edu/abs/2017ApJS..232...11T} {232, 11}

\bibitem[\protect\citeauthoryear{{Tohline} \& {Osterbrock}}{{Tohline} \& {Osterbrock}}{1976}]{tohline_osterbrock_1976}
{Tohline} J.~E.,  {Osterbrock} D.~E.,  1976, \mn@doi [\apjl] {10.1086/182317}, \href {https://ui.adsabs.harvard.edu/abs/1976ApJ...210L.117T} {210, L117}

\bibitem[\protect\citeauthoryear{{Tonry} et~al.,}{{Tonry} et~al.}{2018}]{tonry_denneau_2018_atlas}
{Tonry} J.~L.,  et~al., 2018, \mn@doi [\pasp] {10.1088/1538-3873/aabadf}, \href {https://ui.adsabs.harvard.edu/abs/2018PASP..130f4505T} {130, 064505}

\bibitem[\protect\citeauthoryear{{Vanden Berk} et~al.,}{{Vanden Berk} et~al.}{2004}]{vanden_berk_wilhite_2004}
{Vanden Berk} D.~E.,  et~al., 2004, \mn@doi [\apj] {10.1086/380563}, \href {https://ui.adsabs.harvard.edu/abs/2004ApJ...601..692V} {601, 692}

\bibitem[\protect\citeauthoryear{{Vazdekis}, {Koleva}, {Ricciardelli}, {R{\"o}ck}  \& {Falc{\'o}n-Barroso}}{{Vazdekis} et~al.}{2016}]{vazdekis_2016_emiles_host}
{Vazdekis} A.,  {Koleva} M.,  {Ricciardelli} E.,  {R{\"o}ck} B.,   {Falc{\'o}n-Barroso} J.,  2016, \mn@doi [\mnras] {10.1093/mnras/stw2231}, \href {https://ui.adsabs.harvard.edu/abs/2016MNRAS.463.3409V} {463, 3409}

\bibitem[\protect\citeauthoryear{{V{\'e}ron-Cetty} \& {V{\'e}ron}}{{V{\'e}ron-Cetty} \& {V{\'e}ron}}{2010}]{veroncetty_veron_2010}
{V{\'e}ron-Cetty} M.-P.,  {V{\'e}ron} P.,  2010, \mn@doi [\aap] {10.1051/0004-6361/201014188}, \href {https://ui.adsabs.harvard.edu/abs/2010A&A...518A..10V} {518, A10}

\bibitem[\protect\citeauthoryear{{V{\'e}ron-Cetty}, {Joly}  \& {V{\'e}ron}}{{V{\'e}ron-Cetty} et~al.}{2004}]{veron_cetty_2004_feii_temp}
{V{\'e}ron-Cetty} M.~P.,  {Joly} M.,   {V{\'e}ron} P.,  2004, \mn@doi [\aap] {10.1051/0004-6361:20035714}, \href {https://ui.adsabs.harvard.edu/abs/2004A&A...417..515V} {417, 515}

\bibitem[\protect\citeauthoryear{{Vestergaard} \& {Peterson}}{{Vestergaard} \& {Peterson}}{2006}]{vestergaard_peterson_2006}
{Vestergaard} M.,  {Peterson} B.~M.,  2006, \mn@doi [\apj] {10.1086/500572}, \href {https://ui.adsabs.harvard.edu/abs/2006ApJ...641..689V} {641, 689}

\bibitem[\protect\citeauthoryear{{Wang} \& {Woo}}{{Wang} \& {Woo}}{2024}]{wang_woo_2024}
{Wang} S.,  {Woo} J.-H.,  2024, \mn@doi [\apjs] {10.3847/1538-4365/ad74f2}, \href {https://ui.adsabs.harvard.edu/abs/2024ApJS..275...13W} {275, 13}

\bibitem[\protect\citeauthoryear{{Wang} et~al.,}{{Wang} et~al.}{2019}]{wang_shen_2019}
{Wang} S.,  et~al., 2019, \mn@doi [\apj] {10.3847/1538-4357/ab322b}, \href {https://ui.adsabs.harvard.edu/abs/2019ApJ...882....4W} {882, 4}

\bibitem[\protect\citeauthoryear{{Wang} et~al.,}{{Wang} et~al.}{2025}]{wang_lin_2025}
{Wang} Y.,  et~al., 2025, \mn@doi [Science Advances] {10.1126/sciadv.ady9068}, \href {https://ui.adsabs.harvard.edu/abs/2025SciA...11y9068W} {11, 25.9068}

\bibitem[\protect\citeauthoryear{{Winkler}}{{Winkler}}{1992}]{winkler_1992}
{Winkler} H.,  1992, \mn@doi [\mnras] {10.1093/mnras/257.4.677}, \href {https://ui.adsabs.harvard.edu/abs/1992MNRAS.257..677W} {257, 677}

\bibitem[\protect\citeauthoryear{{Wisotzki}, {Christlieb}, {Bade}, {Beckmann}, {K{\"o}hler}, {Vanelle}  \& {Reimers}}{{Wisotzki} et~al.}{2000}]{wisotzki_christlieb_2000}
{Wisotzki} L.,  {Christlieb} N.,  {Bade} N.,  {Beckmann} V.,  {K{\"o}hler} T.,  {Vanelle} C.,   {Reimers} D.,  2000, \mn@doi [\aap] {10.48550/arXiv.astro-ph/0004162}, \href {https://ui.adsabs.harvard.edu/abs/2000A&A...358...77W} {358, 77}

\bibitem[\protect\citeauthoryear{{Wolf} et~al.,}{{Wolf} et~al.}{2018}]{wolf_onken_2018_smss}
{Wolf} C.,  et~al., 2018, \mn@doi [\pasa] {10.1017/pasa.2018.5}, \href {https://ui.adsabs.harvard.edu/abs/2018PASA...35...10W} {35, e010}

\bibitem[\protect\citeauthoryear{{Wolf}, {Golding}, {Hon}  \& {Onken}}{{Wolf} et~al.}{2020}]{wolf_golding_2020}
{Wolf} C.,  {Golding} J.,  {Hon} W.~J.,   {Onken} C.~A.,  2020, \mn@doi [\mnras] {10.1093/mnras/staa2794}, \href {https://ui.adsabs.harvard.edu/abs/2020MNRAS.499.1005W} {499, 1005}

\bibitem[\protect\citeauthoryear{{Xie}, {Shao}, {Shen}, {Liu}  \& {Li}}{{Xie} et~al.}{2016}]{xie_shao_2016}
{Xie} X.,  {Shao} Z.,  {Shen} S.,  {Liu} H.,   {Li} L.,  2016, \mn@doi [\apj] {10.3847/0004-637X/824/1/38}, \href {https://ui.adsabs.harvard.edu/abs/2016ApJ...824...38X} {824, 38}

\bibitem[\protect\citeauthoryear{{Zaw}, {Chen}  \& {Farrar}}{{Zaw} et~al.}{2019}]{zaw_chen_2019}
{Zaw} I.,  {Chen} Y.-P.,   {Farrar} G.~R.,  2019, \mn@doi [\apj] {10.3847/1538-4357/aaffaf}, \href {https://ui.adsabs.harvard.edu/abs/2019ApJ...872..134Z} {872, 134}

\bibitem[\protect\citeauthoryear{{Zhang}, {Wang}, {Gaskell}  \& {Dong}}{{Zhang} et~al.}{2013}]{zhang_wang_2013}
{Zhang} K.,  {Wang} T.-G.,  {Gaskell} C.~M.,   {Dong} X.-B.,  2013, \mn@doi [\apj] {10.1088/0004-637X/762/1/51}, \href {https://ui.adsabs.harvard.edu/abs/2013ApJ...762...51Z} {762, 51}

\bibitem[\protect\citeauthoryear{{de Grijp}, {Lub}  \& {Miley}}{{de Grijp} et~al.}{1987}]{deGrijp_lub_1987}
{de Grijp} M.~H.~K.,  {Lub} J.,   {Miley} G.~K.,  1987, \aaps, \href {https://ui.adsabs.harvard.edu/abs/1987A&AS...70...95D} {70, 95}

\makeatother
\end{thebibliography}

